A Review of Digital Learning Environments for Teaching Natural Language Processing in K-12 Education

Natural Language Processing (NLP) plays a significant role in our daily lives and has become an essential part of Artificial Intelligence (AI) education in K-12. As children grow up with NLP-powered applications, it is crucial to introduce NLP concepts to them, fostering their understanding of language processing, language generation, and ethical implications of AI and NLP. This paper presents a comprehensive review of digital learning environments for teaching NLP in K-12. Specifically, it explores existing digital learning tools, discusses how they support specific NLP tasks and procedures, and investigates their explainability and evaluation results in educational contexts. By examining the strengths and limitations of these tools, this literature review sheds light on the current state of NLP learning tools in K-12 education. It aims to guide future research efforts to refine existing tools, develop new ones, and explore more effective and inclusive strategies for integrating NLP into K-12 educational contexts.

==> table-overview-tools.tex <==

{
\centering
\begin{tabular}{|>{\raggedright\arraybackslash}p{3cm}|>{\raggedright\arraybackslash}p{3cm}|>{\raggedright\arraybackslash}p{8cm}|}
\hline
\textbf{Name} & \textbf{Number of articles and references} & \textbf{Summary of the tool} \\
\hline
NLP4ALL & 2 \cite{baglini-hjorth-2021-natural, NaturalLanguageProcesing4All} & NLP tool that enables users to tag and analyze textual data, such as tweets \\
\hline
Cognimates & 1 \cite{druga2018growing} & A platform that allows users to input their data to create text/image classification models, integrated with a block programming interface \\
\hline
eCraft2Learn unified user interface (including Snap! AI blocks) & 4 \cite{kahn2018a,kahn2018ai,alimisis2018stem,alimisis2019kids} & A platform that helps students program robotic artifacts using fabrication and technology. Provides blocks to enable AI cloud services and deep learning functionality. \\
\hline
ML4Kids & 1 \cite{lane_2018} & A tool that introduces machine learning by enabling children to create their own machine learning models for recognizing text, images, numbers, and sounds \\
\hline
Teachable Machine (TM) & 2 \cite{carney2020teachable,toivonen2020co} & A web-based interface that lets users train their own image, audio, or pose-based ML classification models without coding \\
\hline
LearningML & 2 \cite{garcia2020learningml,rodriguez2021evaluation} & A platform that helps students build supervised machine learning models and learn about ML \\
\hline
Convo & 2 \cite{zhu2021teaching,zhu2021creating} & A conversational programming agent used by students to create other conversational AI agents \\
\hline
Zhorai & 1 \cite{lin2020zhorai} & A conversational agent that interacts with young children, using visualizations to teach AI/ML \\
\hline
ConvoBlocks & 4 \cite{van2021teaching,van2019tools,van2021alexa,van2022learning} & A block-based programming interface on MIT App Inventor for students (grades 5-12) to develop conversational agents that run on Amazon-enabled devices \\
\hline
Interactive Word Embeddings (IWE) & 1 \cite{bandyopadhyay2022interactive} & An interactive tool for visually exploring word embeddings, relationships, analogies, and semantics in vector space \\
\hline
Build-a-Bot & 1 \cite{pearce2022build} & An open-source tool for students and teachers to create question-answering chatbots and learn AI through the model creation process, designed for classroom environments \\
\hline
\end{tabular}
}



